Self-Contained Kinematic Calibration of a Novel Whole-Body Artificial Skin for Human-Robot Collaboration

In this paper, we present an accelerometer-based kinematic calibration algorithm to accurately estimate the pose of multiple sensor units distributed along a robot body. Our approach is self-contained, can be used on any robot provided with a Denavit-Hartenberg kinematic model, and on any skin equipped with Inertial Measurement Units (IMUs). To validate the proposed method, we first conduct extensive experimentation in simulation and demonstrate a sub-cm positional error from ground truth data --an improvement of six times with respect to prior work; subsequently, we then perform a real-world evaluation on a seven degrees-of-freedom collaborative platform. For this purpose, we additionally introduce a novel design for a stand-alone artificial skin equipped with an IMU for use with the proposed algorithm and a proximity sensor for sensing distance to nearby objects. In conclusion, in this work, we demonstrate seamless integration between a novel hardware design, an accurate calibration method, and preliminary work on applications: the high positional accuracy effectively enables to locate distributed proximity data and allows for a distributed avoidance controller to safely avoid obstacles and people without the need of additional sensing.

==> 2c_collision_avoidance.tex <==
\section{Collision Avoidance}
\kw{May need to remove this entire section}. 


We present a novel collision avoidance algorithm that utilizes proximity sensors embedded within each SU to avoid obstacles. Our method is similar to that of \cite{flacco2012depth}, \cite{flacco2015depth}, and \cite{roncone2016peripersonal} in that all approaches apply a repulsive force to the point on the robot closest to contacting an object. In \cite{flacco2012depth}, the authors use a camera mounted at a third person viewpoint of the robot in order to calculate distance and apply the repulsive force. A camera mounted far from the robot is prone to occlusion and requires overhead calculations to determine the distance between an object and robot. In this section, we demonstrate the capabilities of our calibrated SUs to avoid objects.

\subsection{Repulsive Force}
We utilize the calibrated SU location to apply a force ($\vec{\beta}$) normal to the point the SU is located on the robot body. This alters the trajectory ($\vec{T}$) of the robot such that:
$$\vec{T}\textsubscript{final} = \vec{T} + \vec{\beta}$$

When a measurement from the proximity sensor is received we use the following exponential function to determine the amount of force that should be applied to avoid an object. 

$$
\vec{\beta}=\left\{\begin{array}{ll}\textit{e}^{\frac{-d}{500}}, & \text { if } d < 500 \\ 0, & \text { otherwise }\end{array}\right.
$$

Where \textit{d} is the distance from the proximity sensor in millimeters. \cref{fig:panda}(b) illustrates how $\vec{\beta}$ effects a predetermined trajectory using a Cartesian velocity controller. The force exerted by $\vec{\beta}$ decays exponentially as \textit{d} increases. This causes the robot to rapidly move away from close objects, but still keep a safe distance from those further away.



==> 5_discussion.tex <==
\section{Discussion}\label{sec:discussion}

In our algorithm, we proposed a more accurate computation method for estimating SU acceleration and formulated the optimization problem into two steps: orientation optimization and position optimization. This has led to high performance and resulted in the significant difference between the conventional method. 

==> acknowledgment.tex <==
\section*{ACKNOWLEDGMENT}

Thanks to Alessandro

==> notations.tex <==
\section{Notations}\label{notations}

Accelerometer Measurements
$$ \vec{a} = \{ a_x, \ a_y, \ a_z \} $$

Accelerometer - Measured
$$ \vec{a}^{\text{measured}} = {}^{\text{SU}}\vec{a}^{\text{measured}}$$
$$ \vec{a}^{\text{measured}}_k = {}^{\text{SU}_k}\vec{a}^{\text{measured}}_k $$


Accelerometer - Model
$$ \vec{a}^{\text{model}} = {}^{\text{SU}}\vec{a}^{\text{model}} $$
$$ \vec{a}^{\text{model}}_k = {}^{\text{SU}_k}\vec{a}^{\text{model}}_k $$

\vspace{1cm}

Joints
$$ n = {1, \ \cdots, \ N} $$
$$ J = \{ j_1, \ j_2, \cdots, j_N \} $$
    
Joint Angles

for arbitrary $n$
$$ \vec{\psi}_{j_{1:n}} = \{ \psi_{j_1}, \ \psi_{j_2}, \ \cdots \psi_{j_n} \}$$

for fixed $N$
$$ \vec{\psi}_{j_{1:N}} = \{ \psi_{j_1}, \ \psi_{j_2}, \ \cdots \psi_{j_N} \}$$

Joint angle, velocity and acceleration

$ \{ \psi, \omega, \dot{\omega} \} $ OR 
$ \{ \psi, \dot{\psi}, \ddot{\psi} \} $ OR
$ \{ \psi, \omega, \alpha \} $

\vspace{1cm}

DH Parameters
$$ \Theta = \{ \Theta_{position}, \ \Theta_{orientation} \} = \{ \theta, \ d, \ a, \ \alpha, \ \theta_{acc}, \ d_{acc} \}$$

$$ \Theta_{position} = \{ d, \ a, \ d_{acc} \}$$
$$ \Theta_{orientation} = \{ \theta, \ \alpha, \ \theta_{acc} \}$$


DH Parameters for each SU$_k$ where $k = \{ 1, \ 2, \cdots, K \}$

$$ \Theta_k = \{ \Theta_{\text{position}, k}, \ \Theta_{\text{orientation}, k} \} $$

$$ \Theta_k = \{ \Theta_{\text{pos}, k}, \ \Theta_{\text{orient}, k} \} $$

\begin{alignat}{3}
    \centering
    & \Theta_{\text{orient}, k} && = && \argmin_{\tilde{\Theta}_{\text{orient}, k}} E_s(\tilde{\Theta}_{\text{orient},k}, \  {}^{\text{SU}_k}\vec{a}_{\text{static}}^{\text{measured}}) \nonumber \\
    & \Theta_{\text{position},k} && = && \argmin_{\tilde{\Theta}_{\text{position}, k}} E_d(\tilde{\Theta}_{\text{position},k}, \Theta_{\text{orient},k}, {}^{\text{SU}_k}\vec{a}_{\text{dynamic}}^{\text{measured}}, \psi_k, \dot{\psi}_k) \nonumber
\end{alignat}

\begin{alignat}{3}
    \centering
    & \Theta_{\text{orient}, k} && = && \argmin_{\tilde{\Theta}_{\text{orient}, k}} E_s({}^{j_n}\underline{T}_{\text{SU}_k}(\tilde{\Theta}_k), \  {}^{\text{SU}_k}\vec{a}_{\text{static}}^{\text{measured}}) \nonumber \\
    & \Theta_{\text{pos},k} && = && \argmin_{\tilde{\Theta}_{\text{pos}, k}} E_d({}^{j_n}\underline{T}_{\text{SU}_k}(\tilde{\Theta}_k), {}^{\text{SU}_k}\vec{a}_{\text{dynamic}}^{\text{measured}}, \psi_k, \dot{\psi}_k) \nonumber
\end{alignat}

\vspace{1cm}


Transformation Matrix

$$ \underline{T}  $$


\begin{equation}
\centering
{}^{i}\underline{T}_{i+1} = 
    \Biggl[ \begin{array}{c|c}
      {}^{i}\underline{R}_{i+1} & {}^{i}\vec{r}_{i+1} \\
      \hline
      \vec{0} & 1 \\
    \end{array} \Biggr] \nonumber
\end{equation}

\begin{equation}
    {}^{j_n}{T}_{SU_k} = {}^{j_n}{T}_{v_{n,k}}(d, \theta, a, \alpha) \cdot {}^{v_{n,k}}{T}_{SU_k}(d_{acc},\theta_{acc},0,0)  \nonumber
\end{equation}
